Denoising Multi-modal Sequential Recommenders with Contrastive Learning

There is a rapidly-growing research interest in engaging users with multi-modal data for accurate user modeling on recommender systems. Existing multimedia recommenders have achieved substantial improvements by incorporating various modalities and devising delicate modules. However, when users decide to interact with items, most of them do not fully read the content of all modalities. We refer to modalities that directly cause users' behaviors as point-of-interests, which are important aspects to capture users' interests. In contrast, modalities that do not cause users' behaviors are potential noises and might mislead the learning of a recommendation model. Not surprisingly, little research in the literature has been devoted to denoising such potential noises due to the inaccessibility of users' explicit feedback on their point-of-interests. To bridge the gap, we propose a weakly-supervised framework based on contrastive learning for denoising multi-modal recommenders (dubbed Demure). In a weakly-supervised manner, Demure circumvents the requirement of users' explicit feedback and identifies the noises by analyzing the modalities of all interacted items from a given user.

==> sections/Rebuttal.tex <==
\section{General response}
There is a rapidly-growing research interest in engaging users with multi-modal data for accurate user modeling on recommender systems. Existing multimedia recommenders have achieved substantial improvement by incorporating various modalities and devising delicate modules. However, little research in the literature has investigated the noise modalities/items that appear in the users' interaction sequence. The existence of them will influence the accuracy of users' interests modeling. To this end, we propose a contrastive learning framework for denoising multi-modal recommendation (abbreviated as Demure) by learning user representations that are less affected by noises and more relying on point-of-interests in both the modalities and the item level. Specifically, Demure augments the original user behavior sequences by identifying critical modalities/interactions and accordingly adapting these components to obtain positive/negative multi-modal behavior sequences. Contrastive learning objectives are designed based on the positive/negative user representations obtained from the augmented behavior sequences. Through extensive experiments, we show the Demure framework not only significantly improves the performance of recommendation but also provides an explanation of the motivation of users' interactions.

